Space-Efficient Random Walks on Streaming Graphs

Graphs in many applications, such as social networks and IoT, are inherently streaming, involving continuous additions and deletions of vertices and edges at high rates. Constructing random walks in a graph, i.e., sequences of vertices selected with a specific probability distribution, is a prominent task in many of these graph applications as well as machine learning (ML) on graph-structured data. In a streaming scenario, random walks need to constantly keep up with the graph updates to avoid stale walks and thus, performance degradation in the downstream tasks. We present Wharf, a system that efficiently stores and updates random walks on streaming graphs. It avoids a potential size explosion by maintaining a compressed, high-throughput, and low-latency data structure. It achieves (i) the succinct representation by coupling compressed purely functional binary trees and pairing functions for storing the walks, and (ii) efficient walk updates by effectively pruning the walk search space. We evaluate Wharf, with real and synthetic graphs, in terms of throughput and latency when updating random walks. The results show the high superiority of Wharf over inverted index- and tree-based baselines.

==> list-of-elements.tex <==
%!tex root=main.tex

\section{List of pending elements}
\label{sec:list-of-elements}

\begin{enumerate}
    \item Mini-batched walk update
    
    \item \st{Range Search in walk-trees.} \st{Include space required for caching min/max for each walk-tree. Verify the $v^{next}_{min}$ and $v^{next}_{max}$ of each walk-tree.}
    
    \item Optimization on updating random walks generated from DeepWalk specifically.
    
    \item Policies (?) - two is fine
\end{enumerate}

% Flow of the paper:

% \begin{enumerate}
%     \item How to represent a walk? Walk Triplets
%     \item How to update a walks? Policies
%     \item Batch graph updates or not?
%     \item Graph updates and Walk updates
%     \item Then, use an external data structure such as a Naive Inverted Index $NII$
%     \item Then, it is better to utilize a structure that stores the walks internally within the graph, so that as soon as a graph update arrives we can directly spot which walks are \textcolor{red}{affected} Uncompressed Triplet-based Inverted Index ($UTII$)
%     \item Need compression except for efficiency (Challenge 1). Therefore, we propose the $CW$-trees. We have to make sure we remain efficient; in the worst-case as efficient as the $UTII$. This is directly related to the efficiency of the $CW$-tree operations and specifically the search one. Our idea is to prune the search space when looking for a walk triplet $t$ inside a $CW$-tree by leveraging the ordering properties of pairing functions (range searching and pruning)
% \end{enumerate}

\begin{itemize}
    \item \st{Range Searching. Minimize the search range when searching for a walk triplet inside a $CW$-tree using the ordering properties of the pairing functions (we utilize Szudzik).
    To narrow down the search space even more, i.e.,~construct a range $[lb^{*}, ub^{*}] \subseteq [lb, ub]$. 
    Specifically, we maintain the $min(v_{next}^w)$ and the $max(v_{next}^w)$ the walk-tree of each distinct vertex.}
    
    \item \st{Parallelize Wharf. To achieve that you should do the following:}
        \begin{itemize}
            \item Optimize the the parallel BWU algorithm
            \item \st{Use the green/blue pattern to guard the $MAN$}
            \item \st{Switch all the stl::map entries to the parallel hashmaps that have the same APIs.}
            \item \st{Enable parallelism in the batch walk update.}
        \end{itemize}
    
    \item Streamline the batch strategy to alleviate the potential high memory footprint of the $D_{acc}$ and $I_{acc}$. Utilize double or ring buffers. 
    $D_{acc}$ and $I_{acc}$ are global to all threads. 
    Therefore, a concurrent \textit{lock-free} such as cuckoo hash table must be also used for these structures.
    
    \item \st{``Do not touch the same $CW$-tree again''. 
    Build an index on the walk triplets you have checked while searching in a $CW$-tree and do not suited you at the time, but they belong to a walk $w \in MAN$. 
    Therefore, next time you have to search into the same $CW$-tree for triplets of $w$ you will not have to pay the encoding/decoding trade-off. 
    However, building such an index incurs memory overhead (trade-off between memory and running time).}
    
    \item Given a specific walking model $M$, you can prune the \textcolor{red}{affected} random walks in $MAN$ and end up with a set of \textcolor{red}{affected} walks $MAV'$ that is less; hence, shorten the walk update times. 
    In the end, do not forget to apply changes to only a portion of \textcolor{red}{affected} walks, as DeepWalk (i.e. uniform random sampling) does not give all \textcolor{red}{affected} walks the chance to be updated. 
    You know what you mean. do not forget. 
    This is specific to the random walk model $\mathcal{M}_W$. 
    In case the walk model was that of node2vec (i.e. biased second order walks) then this argument would not hold as you have it in your mind now. 
    So, maybe this should be put as an optimization to make the walk update process faster without sacrificing the statistical indistinguishability property.
    
    \item The $MAV$ currently has the $p_{min}$, i.e.,~the minimum \textcolor{red}{affected} positions of the first \textcolor{red}{affected} vertex  in each \textcolor{red}{affected} walk. 
    One extra idea is to maintain the $p_{max}$ for the random walk model $M$ to prune further.
    An extreme case which we should try also is to keep all \textcolor{red}{affected} positions in an \textcolor{red}{affected} walk for the model to have full knowledge and prune optimally.
    
    \item Assuming we have 3 policies, namely 1) fully crop and rewalk from $p_{min}$ of each \textcolor{red}{affected} vertex  in an \textcolor{red}{affected} walk (arxiv19), 2) crop only from $p_{min}$ till $p_{max}$ of an \textcolor{red}{affected} walk; not until the end, and 3) out of all the intervals in $\{p_{min},\dots,p_{max}\}$ crop and rewalk vertices only between \textcolor{red}{some} $\{p_{i},p_{i+1}\}$ intervals in each \textcolor{red}{affected} walk. 
    Ultimately, all the above-mentioned policies refine the corpus and keep it statistical indistinguishable. 
    The distinctive characteristic is their runtimes and the memory needed to maintain all pairs of $\{p_i, n_i\}$ that correspond to an \textcolor{red}{affected} vertex  in an \textcolor{red}{affected} walk. 
    As a future direction, these policies could change online based on the memory budget \wharf has and/or the timeout threshold the user/developer sets for the update of walks operations. 
    For instance, ``high stakes'' might need policies that maintain the indistinguishability property but perform the corpus update as fast as possible (even if they should utilize more memory) because they must refine/produce the new embeddings asap. 
    
    \item  \st{Put walks and edges in a single $C$-tree, i.e.,~integers corresponding to encoded triplets and to neighbouring vertices such that we can achieve \textit{pure piggybacking}\footnote{\textcolor{red}{This approach needs \textsc{Find} operations that efficiently find integers corresponding to edges and to walk triplets. 
    It will surely increase the graph update time and the walk update time. 
    Furthermore, the \textsc{BoundedRangePruning} concept will be less effective and efficient; let aside that it has to somehow distinguish between integers corresponding to triplet and to edges as we do not want to decode (i.e, unpair) the latter ones leading to rubbish triplets and will compromise the soundness of the result.}}. 
    To verify is such direction is meaningful at all, measure the average Graph Update Time (GUT) and the average Walk Update Time (WUT). 
    Specifically, check how larger is WUT over GUT. 
    In case it is $1$-$2$ orders of magnitude larger than fully/purely piggybacking will not make many practical difference. 
    Measure this when \textit{parallelism is on}, i.e.,~I have the cuckoo hashtable\footnote{\url{https://github.com/efficient/libcuckoo}} for Map of affected vertices (MAN) and the concurrent ring buffer\footnote{\url{https://github.com/cameron314/concurrentqueue}} for the pipelining/streamlining of Batch Walk Update (BWU) algorithm.}
    
    \item \st{The most important though, is to make sure that Aspen works properly with $64$-bit integers.} 
    As an extension, we could modify the Aspen's codebase to accept bigints ($128$-bits or more).
    
    \item \st{Enhance compression by using variable-byte encoding in the chunks.} \textcolor{red}{CAUTION} \st{They already use variable byte-codes for compressing the chunks.} 
    Therefore, just consider Elias-Fano for \wharf++.
    More sophisticated encoding schemes such as Elias Gamma~\cite{wiki:elias-gamma} that compresses multiple numbers inside the same byte exist.
    Such codes use bit-level operations, which are in general more inefficient than the ones that operate on a byte-level.
    As a future work, we plan to utilize a quite promising scheme for encoding the chunks called Elias-Fano \cite{sigir14-partitioned-elias-fano, tois17-clustered-elias-fano, cpm17-dynamic-elias-fano}, because it allows updating the chunks \textit{without decompressing them} as well as enables constant time random access. 
    
    \item Enhance the compressed inverted index so that once we spot a vertex of a random walk, we are able to traverse the walk also from right to left direction (for the follow-up paper or the extension of \wharf).
    
    \item Couple \wharf with a graph generator where we can play with the throughput of source and check/verify/prove that \wharf is able to withstand the input's throughput without backpressure.
\end{itemize}
